SMGRL: Scalable Multi-resolution Graph Representation Learning

Graph convolutional networks (GCNs) allow us to learn topologically-aware node embeddings, which can be useful for classification or link prediction. However, they are unable to capture long-range dependencies between nodes without adding additional layers -- which in turn leads to over-smoothing and increased time and space complexity. Further, the complex dependencies between nodes make mini-batching challenging, limiting their applicability to large graphs. We propose a Scalable Multi-resolution Graph Representation Learning (SMGRL) framework that enables us to learn multi-resolution node embeddings efficiently. Our framework is model-agnostic and can be applied to any existing GCN model. We dramatically reduce training costs by training only on a reduced-dimension coarsening of the original graph, then exploit self-similarity to apply the resulting algorithm at multiple resolutions. The resulting multi-resolution embeddings can be aggregated to yield high-quality node embeddings that capture both long- and short-range dependencies. Our experiments show that this leads to improved classification accuracy, without incurring high computational costs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/old_experiments.tex <==
% removed text from earlier version:









To explore the quality of the embeddings obtained using SMGRL, we first compare with the two closest comparison methods: a single-layer GCN, and a coarsened GCN \citep{huang2021scaling}. Figure ~\ref{fig:GraphSAGE_dimension} shows test set macro $F_1$ score on our four datasets, using a reduction ratio of 0.4, and with a variety of embedding dimension. In addition to the full SMGRL approach, we show results obtained by training a classifier on the embeddings from each layer in isolation; note that the embedding for layer 0 corresponds to a coarsened GCN. In addition, we include GraphSAGE which trained and deployed on the original graph. In Appendix~\ref{app:comparison}, we show comparable results holding embeddings dimension fixed and adjusting the reduction ratio (Figure~\ref{fig:GraphSAGE_reduction}), plus analogous results using APPNP instead of GraphSAGE.



We see several interesting patterns here. First, we note that, as found by \citet{huang2021scaling}, learning a GCN on a coarsened graph and then deploying it on the full graph (Level 0) typically does better than the baseline GCN (GraphSAGE); they suggested this is because using the coarsened graph acts as a regularizer, due to limiting the space of possible convolution operators. However, we find that using just the top-level embeddings---i.e., assigning to each node in $\mathcal{G}$ the embeddings obtained for it's ancestor in the coarsened graph---actually perform \textit{better} than the embeddings obtained using the same algorithm on the original graph. We hypothesise that this is due to two reasons. First, since the GCN is trained on the coarsest later, we would expect the embeddings obtained at this resolution to be highly predictive. This alone does not explain why these embeddings outperform embeddings trained on the original graph, leading to our second hypothesis: the lengthscale associated with the coarser graph may be better aligned with the natural variation in labels.

We also find that combining the embeddings from multiple layers using learned weights tends to lead to better predictive performance than any single layer. This is not surprising: we are able to aggregate information across multiple lengthscales. In principle, if a given level of the hierarchy does not contain relevant information, we can learn to downweight embeddings from that level in the final aggregation.



Clearly, incorporating information obtained at multiple levels of granularity can improve performance over a single level of granularity -- whether that level is the original graph, or a single coarsened layer. However, only one level in the hierarchy has embeddings obtained using a GCN trained on that level. A reasonable question to ask might be whether training one GCN per layer, and combining the resulting embedding, does better than our approach. In Table~\ref{tab:gcn_per_layer} we do exactly that: on the Cora dataset, we compare the SMGRL framework with a single GCN learned at the top level, with a variant that learns a separate GCN for each level. When using our standard weighting aggregation scheme, we perform comparably to this variant, for a significantly lower training cost. Note that, when using a simple mean aggregation, we uniformly outperform the separate GCNs. This is because using a single GCN means that the embeddings at the two levels are compatible---they aggregate information in the same manner, so each dimension carries similar information. 


In Figure~\ref{fig:comparison}, we compare against two popular hierarchical graph embedding methods, HARP \citep{chen2018harp} and MILE \citep{liang2021mile}. Both these methods are much more complex than SMGRL, and accordingly had notably higher runtimes. Despite this, we see that SMGRL outperforms both approaches for most settings.


\subsection{SMGRL can capture long-range dependencies}

Learning in a hierarchical manner allows us to capture long-range dependencies. Nodes that are far apart in the original graph will be closer together in the coarsened graph, and so will have more similar embeddings. To test this hypothesis, we consider a synthetic chain dataset where for each class we generate $k$ chains of length $n$, where each node in the chain is connected to its $k$ nearest neighbors. Nodes in the same chain have the same label. We consider a $d$ dimensional feature vector for each node in the dataset that was sampled from a Gaussian distribution with mean $0$ and variance $1$. In Figure~\ref{fig:chain_length_comparison}, we have used $k=300$ and $d=128$. We see that SMGRL is more robust when increasing the chain length, and that the reduction ratio has a significant impact on performance. This is because the reduction ratio determines the number of levels in the hierarchy, and so the number of levels that can capture long-range dependencies.



By capturing different views of the graph, SMGRL can facilitate the propagation of information in sparse graphs. To test this hypothesis, we use an Erdős-Rényi graph generator to generate $k$ graphs for each class, where each graph has $n$ nodes and nodes are connected to each other with a probability of $p$. We consider a $d$ dimensional feature vector for each node in the dataset that was sampled from a Gaussian distribution with mean $0$ and variance $1$. In Figure~\ref{fig:erdos_renyi}, we have used $k=5$, $d=128$, and $n=500$. We see that SMGRL has can significantly improve the performance of the baseline GraphSAGE model since it can utilize the information from the coarsened graph. This is because the coarsened graph has a higher density of edges, and so the embeddings at the coarsened level can capture more information about the graph.







\subsection{DMGRL obtains high-quality embeddings}\label{sec:16d_embeddings}



Next, we explore how the embeddings generated using DMGRL on top of a GCN. In each case, we generated 16-dimensional embeddings. Figure~\ref{fig:F1_GCN} shows the Macro F1 score of various GCN algorithms, with and without DMGRL. In addition, we include Macro F1 scores for graph coarsened versions of the GCNs, to include an alternative scalable GCN method. In each plot, we show how test set Macro F1 varies with the fraction of nodes labeled in the training set.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/scores_wrt_training_data.png}
    \caption{Macro F1 score obtained on three different datasets, using variants of two GCN models, with different label fractions in the training data.}
    \label{fig:F1_GCN}
\end{figure}

%[ADD: Figure that is like fig:results\_fraction\_of\_data, but that only %includes:
%\begin{itemize}
%    \item APPNP + DMGRL (black, solid line)
%    \item GraphSAGE-mean + DMGRL (\#DDAA33, solid line)
%    \item GraphSAGE-maxpool + DMGRL (\#BB5566, solid line)
%    \item GraphSAGE-GCN + DMGRL (\#004488, solid line)
%    \item vanilla APPNP (black, dotted line)
%    \item vanilla GraphSAGE-mean (\#DDAA33, dotted line)
%    \item vanilla GraphSAGE-maxpool (\#BB5566, dotted line)
%    \item vanilla GraphSAGE-GCN (\#004488, dotted line)
%    \item graph-coarsened APPNP (black, dashed line)
%    \item graph-coarsened GraphSAGE-mean (\#DDAA33, dashed line)
%    \item graph-coarsened GraphSAGE-maxpool (\#BB5566, dashed line)
%    \item graph-coarsened GraphSAGE-GCN (\#004488, dashed line)
%\end{itemize}
%]

\begin{comment}
Looking at \textit{Cora} (Figure [ADD]), we see that including DMGRL leads to a clear performance gain over the basic GCN. By contrast, the graph-coarsening variants of GCN perform comparably or worse to their non-coarsened counterpart. On \textit{CiteSeer} and \textit{PubMed}, DMGRL does not perform as well as the basic GCN model, which we hypothesise is due to long-range dynamics being less important in this task. [TODO: once the vanilla node2vec etc graphs are done, create a corresponding plot with these + the HARP versions, and see if we can see a similar pattern about hierarchies not helping as much in citeseer and pubmed]


[ADD: Figure that is like fig:results\_fraction\_of\_data, but that only includes:
\begin{itemize}
    \item node2vec + HARP (\#DDAA33, solid line)
    \item DeepWalk + HARP (\#BB5566, solid line)
    \item LINE + HARP (\#004488, solid line)
    \item node2vec (\#DDAA33, dotted line)
    \item DeepWalk (\#BB5566, dotted line)
    \item LINE (\#004488, dotted line)
\end{itemize}
]

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/node2vec.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\end{comment}

\subsection{DMGRL can create information-efficient, very low-dimensional embeddings}

Next, we compare the performance of our framework in very low dimensional embedding settings. In [TBD, table or figure] we compare the Macro $F_1$ scores obtained using each of our comparison methods, when the final embedding dimension is constrained to be smaller than the setting considered in Section~\ref{sec:16d_embeddings}. All experiments use 1\% labeled training data. In addition to the raw $F_1$ scores, we also present the relative performance of DMGRL compared with the corresponding GCN.

In this scenario, we see that, in almost all settings, DMGRL leads to improved performance over the corresponding GCN, suggesting that the representations obtained using DMGRL are more efficient than those obtained using DMGRL. We hypothesize that this is due to incorporating information at multiple resolutions. [TODO add something about LINE etc, or remove them from the comparison]

\begin{figure*}
   \centering

   \begin{subfigure}[t]{.45\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/score_wrt_fraction/cora.png}
      \caption{}\label{fig:fig_a}
   \end{subfigure}
   %
   \begin{subfigure}[t]{.45\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/score_wrt_fraction/citeseer.png}
      \caption{}\label{fig:fig_b}
   \end{subfigure}

   \medskip

   \begin{subfigure}[t]{.45\textwidth}
      \centering
      \vspace{0pt}% set the real top as the top
      \includegraphics[width=\linewidth]{figures/score_wrt_fraction/pubmed.png}
      \caption{}\label{fig:fig_c}
   \end{subfigure}
   %
   \begin{minipage}[t]{.45\textwidth}
      \caption{This figure shows a comparison of Macro $F_1$ score.}
      \label{fig:results_fraction_of_data}
   \end{minipage}
\end{figure*}

[TODO add discussion of concat vs mean vs weighted]


%\subsection{Results}
%\subsubsection{Macro $F_1$ score}
%In Fig. \ref{fig:results_fraction_of_data}, we compared $Macro F_1 score$ for different models with respect to the fraction of labeled data available in training set. In our experiment, we used an embedding dimension of 16.

%\subsubsection{Very low dimensional embedding space}
%Next, we compare the performance of our framework in very low dimensional ebedding settings.

%As you can see in Table \ref{table:dim-comparison}, our framework significantly improves the performance of existing GCN models. In Cora, CiteSeer, and PubMed datasets we can see a gain of up to $184.7\%$, $113.9\%$, and $44.5\%$ respectively.

\begin{table*}
   \centering
   %\caption*{Macro $F_1$ on the \textit{Cora} dataset, with varying embedding dimension}
   \begin{tabular}{cccccc}
      %\hline
      %\textbf{Dataset}                                       & \multicolumn{5}{c|}{\textbf{Cora}}                                                                                     \\
      %\hline
      Embedding Dimension                           & 1                        & 1         & 3         & 4         & 5        \\
      \hline
      GraphSAGE                             & 9.567                            & 11.624           & 15.333           & 17.932           & 18.690          \\
      GraphCoarsening+GraphSAGE    & 7.909                            & 11.232          & 11.120           & 13.551           & 14.540           \\
      DMGRL+GraphSAGE            & \textbf{15.482}                           & \textbf{27.164}           & \textbf{36.592}           & \textbf{40.434}           & \textbf{45.443}           \\
      \textit{DMGRL Gain Over GraphSAGE}                   & \textit{61.827\%}                  & \textit{133.688\%} & \textit{138.648\%} & \textit{125.485\%} & \textit{143.140\%} \\
      %\hline
      %$\textbf{GraphSAGE}_{GCN}$                              & 7.538\%                            & 9.639\%            & 11.553\%           & 13.314\%           & 15.194\%           \\
      %$\textbf{DMGRL}+\textbf{GraphSAGE}_{GCN}$               & 11.391\%                           & 19.079\%           & 25.239\%           & 31.094\%           & 33.808\%           \\
      %\textbf{DMGRL Gain Over GraphSAGE}                      & \textbf{51.114\%}                  & \textbf{97.935\%}  & \textbf{118.462\%} & \textbf{133.543\%} & \textbf{122.508\%} \\
      %\hline
      %$\textbf{GraphSAGE}_{MaxPool}$                          & 6.149\%                            & 7.561\%            & 8.638\%            & 9.683\%            & 12.093\%           \\
      %$\textbf{GraphCoarsening}+\textbf{GraphSAGE}_{MaxPool}$ & 9.174\%                            & 9.793\%            & 15.596\%           & 16.103\%           & 17.181\%           \\
      %$\textbf{DMGRL}+\textbf{GraphSAGE}_{MaxPool}$           & 9.369\%                            & 16.233\%           & 20.446\%           & 27.575\%           & 32.171\%           \\
      %\textbf{DMGRL Gain Over GraphSAGE}                      & \textbf{52.366\%}                  & \textbf{114.693\%} & \textbf{136.698\%} & \textbf{184.777\%} & \textbf{166.029\%} \\
      \hline
      APPNP                                         & 7.801                            & 9.713           & 11.239           & 12.498           & 15.007           \\
      GraphCoarsening+APPNP              & 6.326                            & 6.670            & 7.509            & 8.125            & 7.627            \\
      DMGRL+APPNP                         & 10.951                           & 19.172           & 27.161           & 32.931           & 36.508           \\
      \textit{DMGRL Gain Over APPNP}                          & \textit{40.379\%}                  & \textit{97.384\%}  & \textit{141.667\%} & \textit{163.490\%} & \textit{143.273\%} \\
      %\hline
      %\textbf{HARP-node2vec}                                          & 7.195\%                            & 20.962\%            & 37.101\%           & 42.412\%           & 45.441\%           \\
      %\textbf{HARP-DeepWalk}                                          & 14.626\%                            & 23.184\%            & 28.791\%           & 33.742\%           & 37.905\%           \\
      %\textbf{HARP-LINE}                                          & 6.859\%                            & 23.787\%            & \textbf{37.553}\%           & \textbf{44.196}\%           & 45.406\%           \\
      %\hline
   \end{tabular}
   \caption{Macro $F_1$ on the \textit{Cora} dataset, with varying embedding dimension and 1\% labeled data. To compensate the effect of randomly selecting the labeled data, each reported score is the average score over 100 runs.}
   \end{table*}
   \begin{table*}
   \centering
   %\caption*{Macro $F_1$ on the \textit{Citeseer} dataset, with varying embedding dimension}
   \begin{tabular}{cccccc}
      %\hline
      %\textbf{Dataset}                                       & \multicolumn{5}{c|}{\textbf{CiteSeer}}                                                                                    \\
      %\hline
      Embedding Dimension                            & 1                             & 2        & 4         & 4         & 5        \\
      \hline
      GraphSAGE                             & 9.989                                & 14.217           & 17.055           & 20.089           & 21.691          \\
      GraphCoarsening+GraphSAGE    & 8.285                                & 9.504            & 11.964           & 12.016           & 16.760          \\
      DMGRL+GraphSAGE             & \textbf{14.547}                               & \textbf{22.267}           & \textbf{28.322}           & \textbf{29.398}           & \textbf{30.814}          \\
      \textit{DMGRL Gain Over GraphSAGE}             & \textit{45.900\%}                      & \textit{56.622\%}  & \textit{66.062\%}  & \textit{46.338\%}  & \textit{42.058\%} \\
      %\hline
      %$\textbf{GraphSAGE}_{GCN}$                              & 7.867\%                                & 10.478\%           & 12.448\%           & 15.631\%           & 16.812\%          \\
      %$\textbf{DMGRL}_{\textbf{GraphSAGE}_{GCN}}$             & 13.433\%                               & 18.924\%           & 25.179\%           & 26.377\%           & 28.439\%          \\
      %\textbf{DMGRL Gain Over GraphSAGE}                      & \textbf{70.751\%}                      & \textbf{80.606\%}  & \textbf{102.273\%} & \textbf{68.748\%}  & \textbf{69.158\%} \\
      %\hline
      %$\textbf{GraphSAGE}_{MaxPool}$                          & 5.724\%                                & 6.682\%            & 7.553\%            & 7.603\%            & 10.207\%          \\
      %$\textbf{GraphCoarsening}+\textbf{GraphSAGE}_{MaxPool}$ & 8.962\%                                & 11.974\%           & 13.117\%           & 17.174\%           & 17.448\%          \\
      %$\textbf{DMGRL}+\textbf{GraphSAGE}_{MaxPool}$           & 8.437\%                                & 11.427\%           & 13.782\%           & 16.263\%           & 18.032\%          \\
      %\textbf{DMGRL Gain Over GraphSAGE}                      & \textbf{47.396\%}                      & \textbf{71.011\%}  & \textbf{82.470\%}  & \textbf{113.902\%} & \textbf{76.663\%} \\
      \hline
      APPNP                                       & 7.567                                & 8.992            & 12.005           & 13.396           & 15.089          \\
      GraphCoarsening+APPNP               & 6.040                                & 7.648            & 7.449            & 7.413            & 8.039           \\
      DMGRL+APPNP                         & 12.333                               & 19.167           & 24.826           & 27.149           & 29.261          \\
      \textit{DMGRL Gain Over APPNP}                       & \textit{62.984\%}                      & \textit{113.156\%} & \textit{106.797\%} & \textit{102.664\%} & \textit{93.922\%} \\
      %\hline
      %\textbf{HARP-node2vec}                                          & 10.353                            & \textbf{22.549}            & 26.878           & 27.610           & 28.753           \\
      %\textbf{HARP-DeepWalk}                                          & 10.919                            & 18.659            & 26.546           & 23.757           & 23.995           \\
      %\textbf{HARP-LINE}                                          & 9.782                            & 22.484            & \textbf{30.733}           & \textbf{31.037}           & \textbf{31.919}           \\
      %\hline
   \end{tabular}
   \caption{Macro $F_1$ on the \textit{CiteSeer} dataset, with varying embedding dimension and 1\% labeled data. To compensate the effect of randomly selecting the labeled data, each reported score is the average score over 100 runs.}
   \end{table*}
   \begin{table*}
   \centering
   %\caption*{}
   \begin{tabular}{cccccc}
      %\hline
      %\textbf{Dataset}                                       & \multicolumn{5}{c|}{\textbf{PubMed}}                                                                                 \\
      %\hline
      Embedding Dimension                          & 1                           & 2        & 3        & 4        & 5        \\
      \hline
      GraphSAGE                             & 38.361                            & 52.307          & 63.115          & \textbf{69.509}          & \textbf{71.997}          \\
      GraphCoarsening+GraphSAGE    & 29.893                             & 46.525          & 48.194          & 53.457          & 58.695          \\
      DMGRL+GraphSAGE             & 44.487                             & 60.245          & \textbf{65.947}          & 68.176          & 68.364          \\
      \textit{DMGRL Gain Over GraphSAGE   }                   & \textit{15.969\%}                    & \textit{15.175\%} & \textit{4.487\%}  & \textit{-1.917\%} & \textit{-5.046\%} \\
      %\hline
      %$\textbf{GraphSAGE}_{GCN}$                              & 30.608\%                             & 39.995\%          & 46.724\%          & 54.785\%          & 62.506\%          \\
      %$\textbf{DMGRL}+\textbf{GraphSAGE}_{GCN}$               & 39.340\%                             & 51.864\%          & 58.485\%          & 62.883\%          & 64.320\%          \\
      %\textbf{DMGRL Gain Over GraphSAGE}                      & \textbf{28.528\%}                    & \textbf{29.676\%} & \textbf{25.171\%} & \textbf{14.781\%} & \textbf{2.902\%}  \\
      %\hline
      %$\textbf{GraphSAGE}_{MaxPool}$                          & 21.573\%                             & 26.132\%          & 28.768\%          & 32.020\%          & 39.220\%          \\
      %$\textbf{GraphCoarsening}+\textbf{GraphSAGE}_{MaxPool}$ & 29.245\%                             & 45.198\%          & 53.673\%          & 57.674\%          & 56.946\%          \\
      %$\textbf{DMGRL}_{\textbf{GraphSAGE}_{MaxPool}}$         & 29.392\%                             & 35.196\%          & 39.759\%          & 44.507\%          & 47.768\%          \\
      %\textbf{DMGRL Gain Over GraphSAGE}                      & \textbf{36.244\%}                    & \textbf{34.685\%} & \textbf{38.205\%} & \textbf{38.997\%} & \textbf{21.795\%} \\
      \hline
      APPNP                                        & 31.866                            & 38.477          & 46.669          & 48.509          & 56.579          \\
      GraphCoarsening+APPNP              & 24.038                            & 30.570          & 35.940         & 38.894          & 40.306          \\
      DMGRL+APPNP                         & \textbf{46.071}                             & \textbf{61.219}          & 65.574          & 67.604          & 68.736          \\
      \textit{DMGRL Gain Over APPNP}                          & \textit{44.577\%}                    & \textit{59.105\%} & \textit{40.508\%} & \textit{39.363\%} & \textit{21.486\%} \\
      %\hline
      %\textbf{HARP-node2vec}                                          & 19.493\%                            & 65.642\%            & 69.054\%           & 75.150\%           & 74.626\%           \\
      %\textbf{HARP-DeepWalk}                                          & 43.327\%                            & 52.734\%            & 68.046\%           & 72.055\%           & 72.664\%           \\
      %\textbf{HARP-LINE}                                          & 27.023\%                            & 50.060\%            & 66.960\%           & 73.599\%           & 73.171\%           \\
      %\hline
   \end{tabular}
   \caption{Macro $F_1$ on the \textit{PubMed} dataset, with varying embedding dimension and 1\% labeled data. To compensate the effect of randomly selecting the labeled data, each reported score is the average score over 100 runs.}
   \label{table:dim-comparison}
\end{table*}

%\subsubsection{Scalability}
%Our model is highly scalable. It is optimized to learn representation for large graphs in a distributed environment with no shared memory and no network communication overhead. To demonstrate the scalability of our framework, we trained our model on Erdős–Rényi \citep{erdos1960evolution} with vertex size counting from 500 to 7,000 nodes, edge probability of 0.2, node feature size of 1500, and 5 classes.

%As you can see in Fig. \ref{fig:scalability}, our framework can improve the scalability of existing graph representaion learning models.



==> tex/old_method.tex <==
% Attempt at rewrite below

%Our framework consists of three steps, which we summarize in Algorithm~\ref{alg:dmgrl}. First we create a hierarchical coarsening of our graph, which we use to create multiple subgraphs at different levels of resolution. Each node in the original graph only appears directly at the finest level of resolution; nodes at coarser levels of resolution correspond to subgraphs at the previous level. We elaborate in Section~\ref{sec:hierarchical_partitioning}

%Second, we independently train GCNs on each of these subgraphs, as described in Section~\ref{sec:learn_subgraphs}. The resulting GCNs generate embeddings for each node in the subgraph. This stage of the algorithm is embarassingly parallel \citep{neiswanger2014asymptotically}: each subgraph can be assigned to a worker, and those workers operate entirely independently. 

%Finally, we aggregate the embeddings. Due to the hierarchical nature of our partitioning procedure, each node in the original graph is associated with a subgraph---and hence, and an embedding---at each level of the hierarchy. We discuss several lightweight aggregation schemes in Section~\ref{sec:aggregate}.

%We begin by describing each step in more detail in Sections [add-add], before discussing the advantages of DMGRL in Section [add].

\begin{algorithm} % enter the algorithm environment
\caption{SMGRL} % give the algorithm a caption
\label{alg:dmgrl}
\begin{algorithmic} % enter the algorithmic environment
    \REQUIRE Graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V}=(v_1,\dots, v_{|\mathcal{V}|})$; node features $x = (x_1, \dots, x_{|\mathcal{V}|})$; coarsening algorithm {\sc{part}}; representation learning algorithm {\sc embed}; aggregation method for node features $\text{{\sc agg}}_1$; aggregation method for final representations $\text{{\sc agg}}_2$.
    \STATE$\{\{\mathcal{H}^{\ell}_i\}\}$, $\{\{x^{\ell}_i\}\}$, $\{(r_{i})\}, \{(J_\ell)\}\} \leftarrow \text{{\sc HierarchicalPartition}}(\mathcal{G}, x, \text{{\sc part}}, \text{{\sc agg}}_1)$  // Partition into multi-resolutional subgraphs 
    \STATE $L \leftarrow |(J_\ell)| - 1$ 
    \FOR{$\ell=1, \dots, L$ in parallel} %\COMMENT{In parallel}
        \FOR{$j=1, \dots, J_L$ in parallel}
            \STATE $(\tilde{V}^{(\ell)}_j, \tilde{E}^{(\ell)}_j) \equiv \mathcal{H}^{\ell}_j$ // For each subgraph, at each level of the hierarchy
            \STATE Learn function $\text{{\sc{embed}}}^{(\ell)}_j\left(\tilde{V}^{(\ell)}_j; \mathcal{H}^{(\ell)}_j, \{x_{j'}^{(\ell-1)}: v_{j'}^{(\ell-1)}\in \mathcal{H}_j^{(\ell)}\}\right)$ // Learn local GCN
        \ENDFOR
    \ENDFOR
    \FOR{$i=1,\dots, J_0$}
        \STATE $h_i = \emptyset$
        \FOR{$\ell=1, \dots, L$}
            \STATE $h_i \leftarrow h_i \cup \text{{\sc{embed}}}^{(\ell)}_{r_{i, \ell}}\left(v^{(\ell-1)}_{r_{i, \ell-1}}; \mathcal{H}^{(\ell)}_{r_{i, \ell}},  \{x_{j'}^{(\ell-1)}: v_{j'}^{(\ell-1)}\in \mathcal{H}_j^{(\ell)}\}\right)$ // Gather representations corresponding to $i$th node
        \ENDFOR
        \STATE $\phi_i \leftarrow \text{{\sc agg}}(h_i)$ // Combine multi-level representations
    \ENDFOR
    \STATE \textbf{return} {$\phi_1,\dots, \phi_{|\mathcal{V}|}$}
\end{algorithmic}
\end{algorithm}

\subsection{Hierarchically coarsening and partitioning the graph}\label{sec:hierarchical_partitioning}

We begin by creating a multi-level coarsening of our graph, which allows us to obtain consistent partitions at multiple resolutions. We begin by partitioning our graph $\mathcal{G}$ into subgraphs $\mathcal{H}_j{(1)}$. Any graph partitioning algorithm could be used for this purpose; in our experiments we use the Louvain algorithm \citep{blondel2008fast}. The resulting subgraphs becomes nodes in $\mathcal{G}^{(1)}$, the next layer in the hierarchy, with edges added if the corresponding subgraphs in $\mathcal{G}$ are directly connected.

We repeat this procedure to generate an $L$-level hierarchy, where at each level in the hierarchy, the coarsened graph is partitioned into a sequence of subgraphs. We can label each node $v_i$ in our original graph with a vector $(r_{i, 0}, \dots, r_{i, L})$, where $r_{i,0}=i$ represents the node's location in the original graph, and $r_{i, \ell}$ indicates which subgraph it corresponds to at level $\ell$. We summarize the partitioning procedure in Algorithm~\ref{alg:partition}.

\subsection{Distributed graph representation learning}\label{sec:learn_subgraphs}

Independently, we can learn an embedding space for each sub-graph generated by the partitioning module. In this paper, we use (single-layer) GCNs to learn updating rules for each sub-graph. These rules allow us to generate embeddings for the nodes in our training graph. For the bottom level of the hierarchy, we initialize embeddings using the node features; for higher levels, we aggregate node features from lower levels to initialize the embeddings.


If our test set has nodes not present in the training graph, we can add them to our partition by selecting the bottom-level subgraph that contains the plurality of their direct neighbors. We can then use the per-subgraph message passing algorithms to generate embeddings for both new and existing nodes. We note, however, that non-GCN embedding methods could also be used. Indeed, since we treat each subgraph independently, we could dynamically chose different graph representation learning methods for each subgraph. To the best of our knowledge, no graph representation learning framework has been suggested to allow for different learning methods on a different part of the graph.

Since the representations for each subgraph are learned independently, both the memory and the computational requirements of this stage are much lower than those of applying a GCN to the full dataset. From a memory point of view, treating the subgraphs as independent limits the number of nodes each worker must represent. Let $M<<|\mathcal{V}|$ be the size of the largest subgraph generated in our hierarchical partitioning algorithm.\footnote{The exact relationship between $M$ and $|\mathcal{V}|$ will depend on the topology of the graph and on our choice of partitioning algorithm.} In a standard minibatched GCN implementation, a randomly selected minibatch must be augmented with its neighborhood, which could be arbitrarily large. However, in DMGRL, we ignore any edges outside the subgraph, meaning that the number of instantiated nodes is bounded by $M$. 

Ignoring edges that leave the subgraph also reduces the computational complexity. Each sub-graph has a maximum of $M^2$ edges, meaning that the computational cost of running a GCN on a single subgraph is at most $O(M^3)$. Since the sub-graph-specific representations can be learned in parallel, this leads to dramatic speed-ups over a standard GCN implementation.


The hierarchical structure used by DMGRL allows us to capture both long- and short-range dependencies within the graph, without relying on multiple convolutional layers. As we will see in Section [add], this leads to more informative embeddings, when assessed on classification tasks. However, by learning embeddings for each subgraph independently, we avoid the computational cost of fully connected hierarchical approaches, such as HARP or [add some things once the background is complete]. Further, since the embeddings at each subgraph are the result of independently learned message-passing algorithms, differences between the message-passing algorithms provide implicit positional information: proximal nodes will tend to have embeddings generated using the same sequence of message-passing algorithms.

\subsection{Aggregating the multi-resolutional embeddings}\label{sec:aggregate}
As discussed in Section~\ref{sec:hierarchical_partitioning}, each node $v_i$ is associated with a vector $r_i$, which allows us to determine which nodes, in which subgraphs, contain a coarsening of $v_i$. This allows us to select the $L$ embeddings associated with $v_i$, which we then combine into a single embedding.

A number of aggregation techniques can be used to combine the embeddings. Concatenation allows us to preserve all the information in the level-specific embeddings; however it also increases the storage requirements by creating length-$d\cdot L$ embeddings. Mean aggregation does lose some information, but allows us to retain size-$d$ embeddings. 

Alternatively, we could aggregate using a weighted mean, and learn an optimal set of weights for our classification task. This allows us to reduce the information loss, while still retaining compact embeddings. However, it does come at an additional cost, since the weights must be learned in a post-hoc manner. In Section [add], we will see that, while concatenation and weighted mean aggregation do perform better than simple mean aggregation, the performance gap is small, leading us to recommend the mean embedding when both compute and storage are limited.


\subsection{Application in a federated setting}
In many real-world scenarios, data is not stored centrally, but instead is distributed across multiple locations. In the context of graph-structured data, this partitioning is likely to reflect some sort of local structure. For example, in a road traffic network, information may be stored regionally. In an email interaction network, different companies or departments may store information associated with their employees. If the information associated with nodes contains sensitive data, the entities storing that data---which we will refer to as silos---may be reluctant to share this with the rest of the graph.

DMGRL is well-suited to such a siloed setting. Since each silo is likely to contain a highly connected subgraph, we can substitute the hard-coded partitioning implied by the silos, for the bottom level partitioning in Algorithm~\ref{alg:partition}. The representations at this bottom level can be learned within the silos, and need not be sent to a central processor. Instead, each silo communicates a list of other silos to which it is connected, and if appropriate an aggregated vector of covariates to serve as an initial embedding.\footnote{Such an embedding could be privatized using differentially private aggregation mechanisms such as the Laplace mechanism \citep{dwork2006calibrating}.} The central processor can then provide higher-level hierarchical coarsening, and coordinate learning the corresponding embeddings. Once these higher-level embeddings are obtained, the individual silos can combine them with their base-level embeddings.


\subsection{Computational complexity}
As mentioned in Section~\ref{sec:learn_subgraphs}, learning the independent, subgraph-specific representations has computational complexity $O(M^3)$, assuming the largest subgraph is dense and has $M$ nodes. The computational cost of generating the hierarchical partitioning will depend on the complexity of the graph partitioning algorithm used. In our experiments, we used the Louvain algorithm. While this algorithm has theoretical worst-case complexity of $O(|\mathcal{E}|)$, in practice complexity is typically observed to be $O(|\mathcal{V}|\log |\mathcal{V}|)$, and faster variants have been developed that are $O(|\mathcal{V}|\log D)$, where $D$ is the average degree \citep{traag2015faster}. Assuming embeddings are stored in a look-up table and mean aggregation is used, the aggregation step can be carried out in $O(L|\mathcal{V}|)$.

The embarassingly parallel nature of our algorithm means that communication costs can be minimized. Further performance gains can be used by using GCN implementations that make use of GPU computing [add cite].


\begin{algorithm} % enter the algorithm environment
\caption{{\sc HierarchicalPartition}} % give the algorithm a caption
\label{alg:partition}
\begin{algorithmic} % enter the algorithmic environment
    \REQUIRE Graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V}=(v_1,\dots, v_{|\mathcal{V}|})$; node features $(x_1,\dots, x_{|\mathcal{V}|})$; partitioning algorithm {\sc{part}}; aggregation function $\text{{\sc{agg}}}_1$.
    \STATE $\mathcal{V}^{(0)}\leftarrow \mathcal{V}, \mathcal{E}^{(0)}\leftarrow \mathcal{E}, \mathcal{G}^{(0)}\leftarrow (\mathcal{V}^{(0)}, \mathcal{E}^{(0)}), \mathcal{X}^0\leftarrow \mathcal{X}$
    \STATE $\ell \leftarrow 0, J_0 \leftarrow |\mathcal{V}|$
    \FOR{$i=1,\dots, J_0$}
        \STATE $r_{i, 0} \leftarrow i$ // Initialize node label to node id
        \STATE $x_i^{(0)}\leftarrow x_i$
    \ENDFOR
    \WHILE{$\mathcal{G}^{(\ell-1)}$ can be further partitioned}
        \STATE $\ell \leftarrow \ell+1$
        \STATE $\mathcal{H}_1^{(\ell)}, \dots, \mathcal{H}_{J_{\ell}}^{(\ell)} \leftarrow \text{{\sc{part}}}\left(\mathcal{G}^{(\ell-1)}\right)$ // partition graph
        \STATE $\mathcal{V}^{(\ell)} \leftarrow \{v_1^{(\ell)},\dots, v_{J_{\ell}}^{(\ell)}\}$ // Create coarsened graph, with one node per subgraph
        \FOR{$j =1,\dots, J_\ell$}
            \STATE $x_j^{(\ell)} = \text{{\sc agg}}_1\left(\{x_{j'}^{(\ell-1)}: v_{j'}^{(\ell-1)} \in \mathcal{H}_j^{(\ell)}\right)$
        \ENDFOR
        \STATE $\mathcal{E}^{(\ell)} \leftarrow \left\{ (v_i, v_j) \in (\mathcal{V}^{(\ell)}, \mathcal{V}^{(\ell)}): \exists (s, t)\in \mathcal{E}^{(\ell-1)} \text{ s.t. } v_{s}^{(\ell-1)}\in \mathcal{H}_i^{(\ell)}, v_{t}^{(\ell-1)}\in \mathcal{H}_j^{(\ell)}\right\}$
        \STATE $\mathcal{G}^{(\ell)} \leftarrow \left(\mathcal{V}^{(\ell)}, \mathcal{E}^{(\ell)}\right)$
        \FOR{$i=1,\dots, J_0$} 
            \STATE $r_{i, \ell} \leftarrow j: v_{r_{i, \ell-1}}^{(\ell-1)}\in \mathcal{H}_j^{(\ell)}$ // Add id of appropriate graph partition, to each node in the original graph
        \ENDFOR
    \ENDWHILE
    \STATE $\mathcal{H}^{(L)}\leftarrow \mathcal{G}^{(L)}$  // Top level has a single subgraph
    \FORALL{$i=1,\dots, J_0$} 
        \STATE $r_{i, \ell} \leftarrow 1$ // Add id of appropriate graph partition, to each node in the original graph
    \ENDFOR
    \STATE \textbf{return} $\{\{\mathcal{H}^{(\ell)}_i\}_{i=1}^{J_{\ell+1}}\}_{\ell=1}^{L}$, $\{\{x^{(\ell)}_i\}_{i=1}^{J_{\ell+1}}\}_{\ell=1}^{L}$, $\{(r_{i,0}, \dots, r_{i, L})\}_{i=1}^{J_0}, \{(J_0, \dots, J_L)\}\} $
\end{algorithmic}
\end{algorithm}


